Machine Learning Construction: implications to cybersecurity

Statistical learning is the process of estimating an unknown probabilistic input-output relationship of a system using a limited number of observations. A statistical learning machine (SLM) is the algorithm, function, model, or rule, that learns such a process; and machine learning (ML) is the conventional name of this field. ML and its applications are ubiquitous in the modern world. Systems such as Automatic target recognition (ATR) in military applications, computer aided diagnosis (CAD) in medical imaging, DNA microarrays in genomics, optical character recognition (OCR), speech recognition (SR), spam email filtering, stock market prediction, etc., are few examples and applications for ML; diverse fields but one theory. In particular, ML has gained a lot of attention in the field of cyberphysical security, especially in the last decade. It is of great importance to this field to design detection algorithms that have the capability of learning from security data to be able to hunt threats, achieve better monitoring, master the complexity of the threat intelligence feeds, and achieve timely remediation of security incidents. The field of ML can be decomposed into two basic subfields: \textit{construction} and \textit{assessment}. We mean by \textit{construction} designing or inventing an appropriate algorithm that learns from the input data and achieves a good performance according to some optimality criterion. We mean by \textit{assessment} attributing some performance measures to the constructed ML algorithm, along with their estimators, to objectively assess this algorithm. \textit{Construction} and \textit{assessment} of a ML algorithm require familiarity with different other fields: probability, statistics, matrix theory, optimization, algorithms, and programming, among others.f

==> Ch02-Sec00-Abstract.tex <==
\title{Machine Learning Assessment: implications to cybersecurity}%
\author{\AUTHOR}%
\institute{\INSTITUTE}%
\maketitle%
\label{ch:MLassessment}


\abstract{%
  This chapter is dedicated to the assessment and performance estimation of machine learning (ML) algorithms, a topic that is equally
  important to the construction of these algorithms, in particular in the context of cyberphysical security design. The literature is
  full of nonparametric methods to estimate a statistic from just one available dataset through resampling techniques, e.g., jackknife,
  bootstrap and cross validation (CV). Special statistics of great interest are the error rate and the area under the ROC curve (AUC)
  of a classification rule. The importance of these resampling methods stems from the fact that they require no knowledge about the
  probability distribution of the data or the construction details of the ML algorithm. This chapter provides a concise review of this
  literature to establish a coherent theoretical framework for these methods that can estimate both the error rate (a one-sample
  statistic) and the AUC (a two-sample statistic). The resampling methods are usually computationally expensive, because they rely on
  repeating the training and testing of a ML algorithm after each resampling iteration. Therefore, the practical applicability of some
  of these methods may be limited to the traditional ML algorithms rather than the very computationally demanding approaches of the
  recent deep neural networks (DNN). In the field of cyberphysical security, many applications generate structured (tabular) data,
  which can be fed to all traditional ML approaches. This is in contrast to the DNN approaches, which favor unstructured data, e.g.,
  images, text, voice, etc.; hence, the relevance of this chapter to this field.%
}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Yousef2021-BookChapter"
%%% End:


==> preamble-pgfplot.tex <==
\usepackage{pgf,pgfplots,pgfplotstable,tikz,tkz-fct}
\usepackage{tikz-timing}[2009/12/09]
\usepackage{float,fp}
\pgfplotsset{compat=1.11}
\pgfplotsset{width=7cm,compat=1.13}\usepgfplotslibrary{statistics}
\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,decorations.pathreplacing,decorations.pathmorphing,shapes,matrix,shapes.symbols,er,backgrounds,decorations.text,spy,automata}

\DeclareSymbolFont{letters}{OML}{cmm}{m}{it}

\DeclareMathOperator{\dist}{\mathbf{dist}}

\DeclareMathOperator{\dom}{\mathbf{dom}}

\DeclareMathOperator{\relint}{\mathbf{relint}}

\DeclareMathOperator{\aff}{\mathbf{aff}}

\DeclareMathOperator{\rank}{\mathbf{rank}}

\DeclareMathOperator{\bd}{\mathbf{bd}}

\DeclareMathOperator{\relbd}{\mathbf{relbd}}

\DeclareMathOperator{\conv}{\mathbf{conv}}

\DeclareMathOperator{\cl}{\mathbf{cl}}

\DeclareMathOperator{\R}{\mathbf{R}}

\DeclareMathOperator{\MSE}{MSE}

\DeclareMathOperator{\RMS}{RMS}

\DeclareMathOperator*{\E}{E}

\DeclareMathOperator*{\Var}{Var}

\DeclareMathOperator*{\Cov}{Cov}

\DeclareMathOperator*{\Corr}{Corr}


==> sectable.tex <==
    \begin{tabular}{ccccccc}
      \toprule
      \textbf{Estimator} & \textbf{Mean} & \textbf{SD} & \textbf{RMS} & \textbf{RMS$_{AM}$} & $\rho$ & \textbf{Size}\\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.6181 & 0.0434 & 0 & 0.0434 & 1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.5914 & 0.0947 & 0.0973 & 0.0984 & 0.2553 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.7012 & 0.0749 & 0.1128 & 0.1119 & 0.2559 & 20\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.6431 & 0.0858 & 0.0906 & 0.0894 & 0.2218 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.8897 & 0.0475 & 0.2774 & 0.2757 & 0.2231  & \\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.6231 & 0.0410 & 0 & 0.0410 & 1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.5945 & 0.0947 & 0.0956 & 0.0990 & 0.2993 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.6991 & 0.0763 & 0.1066 & 0.1077 & 0.3070 & 22\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.6459 & 0.0846 & 0.0863 & 0.0876 & 0.2726 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.8788 & 0.0499 & 0.2615 & 0.2606 & 0.2991& \\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.6308 & 0.0400 & 0 & 0.0400 &1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.5991 & 0.0865 & 0.0897 & 0.0922 & 0.2946 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.6971 & 0.0701 & 0.0961 & 0.0965 & 0.2997 & 25\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.6442 & 0.0817 & 0.0815 & 0.0828 & 0.2758 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.8656 & 0.0471 & 0.2406 & 0.2395 & 0.2833& \\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.6359 & 0.0358 & 0 & 0.0358 &1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.6035 & 0.0840 & 0.0874 & 0.0901 & 0.2904 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.6962 & 0.0688 & 0.0906 & 0.0915 & 0.2934 & 28\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.6479 & 0.0792 & 0.0785 & 0.0802 & 0.2719 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.8554 & 0.0472 & 0.2253 & 0.2246 & 0.2747& \\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.6469 & 0.0343 & 0 & 0.0343 &1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.6170 & 0.0750 & 0.0792 & 0.0807 & 0.2746 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.6997 & 0.0623 & 0.0818 & 0.0817 & 0.2722 & 33\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.6553 & 0.0761 & 0.0752 & 0.0766 & 0.2656 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.8419 & 0.0439 & 0.2010 & 0.1999 & 0.2434& \\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.6571 & 0.0308 & 0 & 0.0308 &1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.6244 & 0.0711 & 0.0753 & 0.0783 & 0.3185 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.6981 & 0.0598 & 0.0710 & 0.0725 & 0.3167 & 40\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.6595 & 0.0739 & 0.0707 & 0.0739 & 0.3092 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.8246 & 0.0431 & 0.1735 & 0.1730 & 0.2923& \\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.6674 & 0.0271 & 0 & 0.0271 & 1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.6357 & 0.0654 & 0.0690 & 0.0727 & 0.3534 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.6995 & 0.0556 & 0.0615 & 0.0642 & 0.3570 & 50\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.6685 & 0.0690 & 0.0646 & 0.0690 & 0.3522 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.8091 & 0.0406 & 0.1473 & 0.1474 & 0.3517& \\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.6808 & 0.0217 & 0 & 0.0217 &1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.6533 & 0.0546 & 0.0602 & 0.0611 & 0.2451 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.7053 & 0.0471 & 0.0527 & 0.0531 & 0.2488 & 66\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.6840 & 0.0568 & 0.0556 & 0.0569 & 0.2477 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.7946 & 0.0355 & 0.1195 & 0.1192 & 0.2499& \\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.6965 & 0.0158 & 0 & 0.0158 & 1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.6738 & 0.0454 & 0.0483 & 0.0507 & 0.3422 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.7119 & 0.0399 & 0.0405 & 0.0428 & 0.3492 & 100\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.7004 & 0.0452 & 0.0426 & 0.0453 & 0.3448 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.7772 & 0.0312 & 0.0860 & 0.0866 & 0.3596& \\
      \midrule
      \multicolumn{1}{l}{$\AUC_{\mathbf{t}}$} & 0.7141 & 0.0090 & 0 & 0.0090 &1.0000 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( \ast\right) }}$} & 0.6991 & 0.0298 & 0.0327 & 0.0334 & 0.2288 & \\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632\right) }}$} & 0.7205 & 0.0272 & 0.0273 & 0.0279 & 0.2291 & 200\\
      \multicolumn{1}{l}{$\widehat{\AUC}_{\mathbf{t}}^{_{\left( .632+\right)}}$} & 0.7170 & 0.0285 & 0.0279 & 0.0286 & 0.2294 & \\
      \multicolumn{1}{l}{$\overline{\AUC}_{\mathbf{t}}$} & 0.7573 & 0.0228 & 0.0487 & 0.0489 & 0.2277 & \\
      \bottomrule
    \end{tabular}


